A Fully Problem-Dependent Regret Lower Bound for Finite-Horizon MDPs

We derive a novel asymptotic problem-dependent lower-bound for regret minimization in finite-horizon tabular Markov Decision Processes (MDPs). While, similar to prior work (e.g., for ergodic MDPs), the lower-bound is the solution to an optimization problem, our derivation reveals the need for an additional constraint on the visitation distribution over state-action pairs that explicitly accounts for the dynamics of the MDP. We provide a characterization of our lower-bound through a series of examples illustrating how different MDPs may have significantly different complexity. 1) We first consider a "difficult" MDP instance, where the novel constraint based on the dynamics leads to a larger lower-bound (i.e., a larger regret) compared to the classical analysis. 2) We then show that our lower-bound recovers results previously derived for specific MDP instances. 3) Finally, we show that, in certain "simple" MDPs, the lower bound is considerably smaller than in the general case and it does not scale with the minimum action gap at all. We show that this last result is attainable (up to $poly(H)$ terms, where $H$ is the horizon) by providing a regret upper-bound based on policy gaps for an optimistic algorithm.

==> 4_discussion_old.tex <==
% !TEX root = main.tex 
\section{Discussion}\label{sec:discussion}

%We now illustrate a series of examples that show some interesting properties of our lower bound.

\input{./mdp_figure}

We briefly recall existing lower bounds. In \emph{ergodic} average-reward MDPs, \citet{burnetas1997optimal,tewari2007opotimistic,ok2018exploration} showed that the optimal problem-dependent regret scales as the sum of the inverse sub-optimality gaps\footnote{To be precise, it scales with the sum of local complexity measures which are related to the action gaps~\cite{tewari2007opotimistic}.}. In finite-horizon MDPs, \citet{simchowitz2019non} first showed that the sum of the inverse gaps is a loose lower bound for a specific family of optimistic algorithms, which in the worst-case may suffer from a regret of at least $S/\Delta_{\min}$. \citet{xu2021fine} later refined this result showing that there exists a ``hard'' MDP where any $\alpha$-good algorithm (Def.~\ref{def:good-alg}) suffers a regret proportional to $SA/\Delta_{\min}$, which is (exponentially)\todompout{potentially?} larger than the sum of inverse gaps by a factor $\frac{Z_{\mathrm{mul}}}{\Delta_{\min}}$, where $Z_{\mathrm{mul}}$ is the total number of optimal actions in states where the optimal action is not unique. This suggests that the number of non-unique optimal actions may be key to characterize the ``worst-case'' complexity of learning in finite-horizon MDPs.

\textbf{On the importance of the dynamics constraint to match existing lower bounds.} 
We consider the MDP $\M$ introduced in~\citep{xu2021fine} (see Fig.~\ref{fig:example-du-variant} with $\kappa=0$) and we define $\mathfrak{M}$ as the set of MDPs with exactly the same dynamics as $\M$ but possibly different rewards, which are assumed to be Gaussian. In this problem $\Delta_{\min} = \epsilon$. We instantiate our lower bound in this case with and without the dynamics constraints.

\begin{corollary}\label{cor:du.example}
	Let $\M$ be the MDP illustrated in Fig.~\ref{fig:example-du-variant} with $\kappa=0$. Let $\wt v(\M)$ the value of the optimization problem of Theorem~\ref{th:main-lower-bound} \textbf{without dynamics constraints}, then $\wt v(\M) = 2(1-\alpha)(H+A-2)/\Delta_{\min} \approxeq \big(\log(S) + A\big)/\Delta_{\min}$. On the other hand, the lower bound in Theorem~\ref{th:main-lower-bound} \textbf{with dynamics constraints} yields $v^\star(\M) \gtrsim SA/\Delta_{\min}$.
\end{corollary}

This result shows that ignoring the dynamics constraints leads to an exponentially loose lower bound.\todompout{exponentially is not clear in this sentence} On the other hand, when computing the original lower bound of Theorem~\ref{th:main-lower-bound} we match the lower bound by~\citet{xu2021fine} for this configuration.

% \textbf{On the usefulness of the policy view.} The policy view of Prop.~\ref{prop:policy-based} is particularly convenient to simplify the expression of the lower bound in some specific cases. One illustrative example is the problem considered above, where all MDPs in $\mathfrak{M}$ share the same dynamics. In this case, the lower bound can be written as
% %
% \begin{equation*}
% 	\begin{aligned}
% 		&\underset{\omega_\pi \geq 0}{\inf}&& \sum_{\pi\in\Pi} \omega_\pi \langle \theta, \phi^\star - \phi^\pi\rangle,
% 		\\
% 		&
% 		\quad \mathrm{s.t.} \quad
% 		&& 
% 		\forall \pi \notin \weakopt(\M) : \|\phi^\pi\|_{D_\omega^{-1}}^2 \leq \frac{\Gamma(\pi)^2}{2(1-\alpha)},
% 	\end{aligned}
% \end{equation*}
% %
% where $\theta \in \mathbb{R}^{SAH}$ is a vector containing all mean rewards, i.e., $\theta_{s,a,h} = r_h(s,a)$, $\phi^\pi \in \mathbb{R}^{SAH}$ is the vector containing the state distribution $\rho_{\M}^\pi$, and $D_\omega := \sum_{\pi\in\Pi} \omega_\pi \mathrm{diag}(\rho_{\M,h}^\pi(s,a)) \in \mathbb{R}^{SAH\times SAH}$ is a diagonal matrix proportional to the number of times each policy is selected. With this notation we have $V_{\M,0}^\pi = \theta^T \phi^\pi$ and $V_{\M,0}^\star = \theta^T \phi^{\star} := \theta^T \phi^{\pi^\star}$ for some optimal policy $\pi^\star$.\footnote{This formulation bears a strong resemblance with the asymptotic lower bound for combinatorial semi-bandit setting. We leave it as a future work to further study the connection and differences between the two settings.} It is then possible to instantiate this expression for Fig.~\ref{fig:example-du-variant} and obtain the statement of Cor.~\ref{cor:du.example}.


\paragraph{On the dependence on the sum of inverse gaps.}

While the lower bound of~\citet{xu2021fine} shows that there exists problem where the regret is much larger than the inverse of the gaps, in the following we derive a result that is somewhat complementary: we show that there exists a large class of MDPs where the lower bound scales as the sum of the action gaps, regardless of the presence of multiple optimal actions.

\begin{proposition}\label{prop:full-support}
Let $\M$ be an MDP satisfying Assumption~\ref{ass:unique-opt-rho} such that $\rho_{\M,h}^\star$ is \emph{full-support} 
%(i.e., strictly positive at all states)
 for all $h\in[H]$ (i.e., $\rho_{\M,h}^\star(s)>0$, $\forall s,h$). Then, 
\begin{align*}
v^\star(\M) = (1-\alpha)\sum_{h\in[H]}\sum_{s\in\S}\sum_{a\in\A} \frac{\Delta_{\M,h}(s,a)}{\mathcal{K}_{s,a,h}(\M)},
\end{align*}
where $\mathcal{K}_{s,a,h}(\M) : = \inf_{\bar{p},\bar{q} \in \Lambda_{s,a,h}(\M)}\big\{ \mathrm{KL}(p_h(s,a), \bar{p}) + \mathrm{KL}(q_h(s,a), \bar{q})\big\}$ and $\Lambda_{s,a,h}(\M) := \{\bar{p}\in\P(\S),\bar{q}\in\P(\mathbb{R}) : \mathbb{E}_{x\sim \bar{q}}[x] + \bar{p}^T V_{\M,h+1}^\star > V_{\M,h}^\star(s)\}$. Moreover,
\begin{align*}
v^\star(\M) \leq (1-\alpha)\sum_{h\in[H]}\sum_{s\in\S}\sum_{a\in\A} \frac{2(H-h)^2}{\Delta_{\M,h}(s,a)}.
\end{align*}
\end{proposition}
Note that the full-support condition for $\rho_{\M,h}^\star$ is weaker than ergodicity for average-reward MDPs since it is required only for the optimal policy and not for all policies. For MDPs with this property, the lower bound is obtained by a \emph{decoupled} exploration strategy similar to the one for ergodic MDPs, where the optimal allocation focuses on exploring sub-optimal actions regardless of how to reach the corresponding state, while the exploration of the state space comes ``for free'' from trying to minimize regret w.r.t.\ the optimal policy itself. Interestingly, this result holds even for $Z_{\mathrm{mul}} > 0$, suggesting that the dependency $\frac{Z_{\mathrm{mul}}}{\Delta_{\min}}$ derived in~\citep{xu2021fine} may be relevant only under specific reachability properties (e.g., when the optimal occupancy measure is not full support).


\paragraph{On the dependence on the minimum gap.}

Regret may not depend on gap min: using a modified version of the instance of~\cite{xu2021fine}, we do not scale with gap min anymore but some other quantity.

Informal statement (to be described)
\begin{proposition}
There exists an MDP $\M$ with $0 < \Delta_{\min} \ll \Delta_{\max}$ where the lower bound of Theorem~\ref{th:abc} yields $v^\star(\M) \lesssim \frac{SA}{\Delta_{\max}}$.
\end{proposition}


\todompout{Should we comment on the fact we consider known dynamics as final comment? e.g. that the dependence on the gap is potentially optimal given the result of~\citep{xu2021fine} and thus it can only increase by poly factors in $S,A,H$?}
